Formal Models of the OSPF Routing Protocol

We present three formal models of the OSPF routing protocol. The first two are formalised in the timed process algebra T-AWN, which is not only tailored to routing protocols, but also specifies protocols in pseudo-code that is easily readable. The difference between the two models lies in the level of detail (level of abstraction). From the more abstract model we then generate the third model. It is based on networks of timed automata and can be executed in the model checker Uppaal.

==> eptcsdata.tex <==
\providecommand{\firstpage}{72}
\providecommand{\publicationstatus}{A. Fehnker and H. Garavel (Eds.):\\
Models for Formal Analysis of Real Systems (MARS 2020)\\
EPTCS 316, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.316.4}{10.4204/EPTCS.316.4}}
\pdfoutput=1

